Better Decomposition, Free Aggregation: A Synthesizer-Folding Framework for Multilingual Multi-Hop Question Answering

Multilingual retrieval-augmented generation (mRAG) equips large language models with access to globally distributed external knowledge for complex multilingual question answering. Recent approaches either translate retrieved documents into English or the query language to bridge the cross-lingual semantic gap, or decompose a complex query into sub-questions and aggregate the intermediate reasoning process. However, both lines of work suffer from two limitations. First, one-size-fits-all translation alignment, blanket translation discards culturally and linguistically native information unique to the target language, introduces translation noise, and inflates system cost. Second, greedy decomposition and aggregation, uncontrolled decomposition produces redundant sub-questions that compound errors during step-wise reasoning, and the final aggregation over reasoning paths further amplifies these errors. We address both with our method Syfer, a synthesizer-folding framework for multilingual multi-hop question answering that defers translation rather than applying it by default. Syfer first invokes a format-constrained decomposer to produce a sub-question graph in the original language, followed by a decomposition-quality check; when the check passes, sub-questions are answered sequentially under a retrieve-then-answer policy in the target language, and the English translation pathway with bilingual sub-question graph alignment is activated only when the check fails. Experiments across multiple languages show that Syfer attains competitive accuracy while striking a favourable balance between performance and computational cost.

==> chapters/03_ProblemFormulation.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\noindent\textbf{Multilingual Retrieval-Augmented Generation.}
A multilingual retrieval-augmented generation system consists of three components: a multilingual document corpus, a retriever, and a generator. Let $\mathcal{L}$ denote the set of supported languages and let
\begin{equation}
  \mathcal{C} \;=\; \{\, d_{1}, d_{2}, \ldots, d_{|\mathcal{C}|} \,\}
  \label{eq:corpus}
\end{equation}
denote the document corpus, where each document $d \in \mathcal{C}$ is written in one of the languages in $\mathcal{L}$. The corpus is shared across all query languages and is not partitioned by language. A user query is a pair $(Q, L)$ with $L \in \mathcal{L}$, where $Q$ may be expressed in any language of $\mathcal{L}$. Given $(Q, L)$, the retriever $\mathcal{R}$
\begin{equation}
  \mathcal{R}\;(Q, L, \mathcal{C})\;\longmapsto\;\mathcal{D}_{Q} \subseteq \mathcal{C}
  \label{eq:retriever}
\end{equation}
% \begin{equation}
%   \mathcal{D}_{Q} \;=\; \mathcal{R}(Q, L, \mathcal{C}) \;\subseteq\; \mathcal{C},
%   \label{eq:retriever}
% \end{equation}
returns a set of supporting documents $\mathcal{D}_{Q}$ deemed most relevant to $Q$, after which the generator $\mathcal{G}$ produces the answer
\begin{equation}
  A \;=\; \mathcal{G}(Q,\, \mathcal{D}_{Q})
  \label{eq:generator}
\end{equation}
conditioned on the query and the retrieved evidence. Note that $\mathcal{D}_{Q}$ may contain documents whose language differs from $L$; this cross-lingual mismatch between the query and the supporting evidence is the core difficulty addressed by mRAG and a primary source of error in this work.

\noindent\textbf{Multilingual Multi-hop Question Answering.}
A query $(Q, L)$ is a multi-hop question when no single document in $\mathcal{C}$ provides sufficient evidence to derive $A$, and the gold supporting evidence is instead distributed across multiple documents. Formally, there exists a set of gold documents
\begin{equation}
  \mathcal{D}_{Q}^{\star} \;=\; \{\, d_{i_{1}}, d_{i_{2}}, \ldots, d_{i_{k}} \,\} \;\subseteq\; \mathcal{C}, \qquad k \,\geq\, 2,
  \label{eq:gold-docs}
\end{equation}
such that $A$ can be derived from $\mathcal{D}_{Q}^{\star}$ but not from any strict subset of size smaller than $k$, where $k$ is referred to as the hop count of $Q$. In the multilingual setting, the gold documents in $\mathcal{D}_{Q}^{\star}$ may belong to different languages and need not share the language $L$ of the query. The system must therefore recover a cross-lingual subset of $\mathcal{C}$ via $\mathcal{R}$ and integrate the evidence under a single coherent reasoning trace via $\mathcal{G}$. The end-to-end task is to learn a function $\mathcal{F}$
\begin{equation}
  \mathcal{F}\;(Q,\, L,\, \mathcal{C}) \;\longmapsto\; A
  \label{eq:task}
\end{equation}
% \begin{equation}
%   A \;=\; \mathcal{F}(Q, L, \mathcal{C}).
%   \label{eq:task}
% \end{equation}
that maximizes answer correctness against a reference answer $A^{\star}$ written in language $L$, evaluated by Exact Match (EM) and token-level F1.


==> chapters/04_Methodology.tex <==
\section{Methodology}
\label{sec:method}

\textsc{Syfer} is organized as a linear flow over four stages (Fig.~\ref{f1}). (1)~\emph{Logical Decomposition Distillation} trains a compact student decomposer from teacher-generated DAG annotations on an independent corpus--query pool. Given an input query $Q$ in language $L$, (2)~\emph{Synthesizer-Folded Decomposition} produces a monolingual sub-question DAG $D_{L}$ in which the terminal sub-question is constrained to be a structural paraphrase of $Q$, folding the classical end-of-pipeline aggregation into the last hop. (3)~\emph{Faithfulness Verification and Bilingual Fallback} measures the cosine similarity between the filled terminal sub-question and $Q$; if it clears a threshold, $D_{L}$ is committed, otherwise $Q$ is translated, an English DAG is decomposed in parallel, and aligned nodes are fused into a bilingual graph $D_{F}$. (4)~\emph{Cross-Lingual Retrieval and Answering} topologically sorts the resulting graph, retrieves from a single multilingual index per hop, removes cross-lingual parallel duplicates with maximal marginal relevance (MMR), and answers in order. Stage~(1) is offline; stages~(2)--(4) form the inference pipeline.

\begin{figure*}[t]
  \centering
  \vspace{-1em}
  \includegraphics[width=\linewidth]{figure/mainfig.pdf}
  \vspace{-2em}
  \caption{Overview of \textsc{Syfer}: synthesizer-folded decomposition, faithfulness verification with bilingual fallback, and cross-lingual retrieval-and-answering.}
  \vspace{-1em}
  \label{f1}
\end{figure*}

\subsection{Logical Decomposition Distillation}
\label{ssec:distill}

A natural alternative is to invoke a frontier LLM to decompose every test query online, but this couples inference cost to the strongest available model and gives no guarantee that the resulting decomposition is suited to synthesizer folding. We instead detach the decomposer from the answering model and shape its behaviour by distillation on a corpus--query pool that is held out from any evaluation data, so that synthesizer folding becomes a learned property rather than a prompt-time hope.

The teacher $M_{T}$ reads each query $Q$ and emits a sub-question DAG $D^{*}$ that is acyclic, exposes a unique terminal node, and uses placeholder tokens $\#i$ to mark cross-node dependencies. The non-trivial requirement is that the filled terminal sub-question $q_{n}^{\text{filled}}$ be a structural paraphrase of $Q$ in the embedding space, formalised by the synthesizer-folding constraint
\begin{equation}
  \cos\!\left(\mathbf{e}(q_{n}^{\text{filled}}),\; \mathbf{e}(Q)\right) \;\geq\; \tau_{\text{constraint}},
  \label{eq:constraint}
\end{equation}
where $\mathbf{e}(\cdot)$ is the retriever embedding. A decomposition is admissible only if its terminal hop, after placeholder substitution, can stand in for $Q$ in retrieval space. Records violating Eq.~\eqref{eq:constraint} under the teacher's own annotations are filtered per language, yielding the supervision $\mathcal{D}_{\text{train}} = \{(Q^{(k)}, D^{*(k)})\}_{k=1}^{N}$.

For each instance, $D^{*}$ is linearised into a token sequence $y = (y_{1}, \ldots, y_{T})$ that preserves node order and edge structure, with the teacher's intermediate sub-answers stripped so that the student learns the shape of a faithful decomposition rather than memorising specific evidence. The student decomposer with parameters $\theta$ is then optimised by minimising the standard token-level cross-entropy loss
\begin{equation}
  \mathcal{L}_{\text{Distill}}(\theta)
  \;=\; -\,\mathbb{E}_{(Q,\,y)\sim \mathcal{D}_{\text{train}}}
  \sum_{t=1}^{T} \log p_{\theta}\!\left(y_{t} \,\middle|\, Q,\, y_{<t}\right),
  \quad
  \theta^{*} \;=\; \arg\min_{\theta}\;\mathcal{L}_{\text{Distill}}(\theta).
  \label{eq:sft-loss}
\end{equation}
The trained $\theta^{*}$ defines the inference-time decomposer in Section~\ref{ssec:syn-fold} and is reused, without branch-specific fine-tuning, by the bilingual fallback in Section~\ref{ssec:faith-fallback}.


\subsection{Synthesizer-Folded Decomposition}
\label{ssec:syn-fold}

Conventional multi-hop RAG pipelines reserve a dedicated aggregation call at the end, asking the model to synthesize the final answer from $(Q, q_{1{:}n}, a_{1{:}n})$. This last call is where most cross-lingual interference accumulates, because the long bilingual reasoning trace forces the generator to disambiguate hop-by-hop noise. \textsc{Syfer} removes this call by shifting the synthesis burden into decomposition: the decomposer produces a terminal sub-question that, once filled, already speaks for $Q$. Concretely, given $Q$ in language $L$,
\begin{equation}
  D_{L} \;=\; \mathrm{Decompose}_{\theta^{*}}(Q),\qquad D_{L} = (V_{L}, E_{L}),
  \label{eq:decompose}
\end{equation}
with $V_{L} = \{q_{1}, \ldots, q_{n}\}$ and $E_{L} \subseteq V_{L} \times V_{L}$. An edge $(q_{i}, q_{j}) \in E_{L}$ indicates that the answer $a_{i}$ is required to instantiate $q_{j}$; substituting $a_{i}$ for each placeholder $\#i$ ($i<j$) in $q_{j}$ yields the filled form $q_{j}^{\text{filled}}$. The graph is acyclic and exposes a unique terminal node $q_{n}$. Trained under Eq.~\eqref{eq:constraint}, the terminal node is no longer an arbitrary leaf but a learned slot whose filled form encodes both $Q$ and the prior sub-answers, so that answering it against the corpus is, by construction, equivalent to aggregating.


\subsection{Faithfulness Verification and Bilingual Fallback}
\label{ssec:faith-fallback}

Eq.~\eqref{eq:constraint} is enforced only at training time, but the trained decomposer occasionally produces a terminal sub-question whose filled form drifts away from $Q$, especially on long or syntactically unusual queries. We therefore turn the training-time constraint into an \emph{inference-time gate}: before retrieval, \textsc{Syfer} checks that the filled terminal still embeds close to $Q$, and only then commits to the monolingual path. This single decision both detects unfaithful decompositions and routes them toward a complementary cross-lingual signal, without any additional verifier model. Formally,
% \begin{equation}
%   \mathrm{score}(D_{L}) = \cos\!\left(\mathbf{e}(q_{n}^{\text{filled}}),\, \mathbf{e}(Q)\right),
%   \quad
%   \mathrm{Route}(D_{L}) =
%   \begin{cases}
%     D_{L}, & \mathrm{score}(D_{L}) \geq \tau_{\text{constraint}}, \\
%     \mathrm{BilingualFallback}(D_{L}, Q), & \mathrm{score}(D_{L}) < \tau_{\text{constraint}},
%   \end{cases}
%   \label{eq:route}
% \end{equation}
\begin{equation}
\begin{aligned}
  \mathrm{score}(D_{L})
  &= \cos\!\left(\mathbf{e}(q_{n}^{\text{filled}}),\, \mathbf{e}(Q)\right), \\
  \mathrm{Route}(D_{L})
  &=
  \begin{cases}
    D_{L}, & \mathrm{score}(D_{L}) \geq \tau_{\text{constraint}}, \\
    \mathrm{BilingualFallback}(D_{L}, Q),
    & \mathrm{score}(D_{L}) < \tau_{\text{constraint}}.
  \end{cases}
\end{aligned}
\label{eq:route}
\end{equation}
sharing the threshold $\tau_{\text{constraint}}$ with training so that the gate inherits its calibration. Translation is therefore not the default but a recovery mechanism scoped to queries the monolingual path cannot cover faithfully.

The fallback injects English signal only where it is needed. The query is translated to its English parallel $Q_{\mathrm{en}}$, and the same distilled decomposer is invoked again to produce $D_{\mathrm{en}} = (V_{\mathrm{en}}, E_{\mathrm{en}})$ with $V_{\mathrm{en}} = \{q_{1}^{\mathrm{en}}, \ldots, q_{m}^{\mathrm{en}}\}$; reusing $\theta^{*}$ keeps the two DAGs comparable in granularity and embedding geometry. We then iteratively pair the most similar cross-lingual nodes,
\begin{equation}
  (q_{i}^{L*}, q_{j}^{\mathrm{en}*}) = \arg\max_{q_{i}^{L} \in V_{L},\, q_{j}^{\mathrm{en}} \in V_{\mathrm{en}}}
  \mathrm{sim}\!\left(\mathbf{e}(q_{i}^{L}),\, \mathbf{e}(q_{j}^{\mathrm{en}})\right),
  \label{eq:node-align}
\end{equation}
accepting only pairs above an alignment threshold $\tau_{\text{align}}$. Each accepted pair upgrades $q_{i}^{L*}$ into a bilingual node carrying both sub-questions, redirects all edges incident to $q_{j}^{\mathrm{en}*}$ to the upgraded node, and removes $q_{j}^{\mathrm{en}*}$ from $V_{\mathrm{en}}$. Iterating until no remaining pair clears $\tau_{\text{align}}$ yields
\begin{equation}
  D_{F} = \mathrm{Fuse}(D_{L}, D_{\mathrm{en}}),
  \label{eq:fused-graph}
\end{equation}
whose node set is exactly $V_{L}$ with some nodes upgraded; in particular, the terminal of $D_{F}$ is inherited from $q_{n}^{L}$, possibly upgraded into the bilingual pair $(q_{n}^{L}, q_{m}^{\mathrm{en}})$. The fused terminal preserves the synthesizer-folding role of $q_{n}^{L}$ and may additionally consult its English counterpart at answer time. If $Q$ is already in English, the fallback is degenerate. The output of this stage is therefore $D_{L}$ or $D_{F}$.


\subsection{Cross-Lingual Retrieval and Answering}
\label{ssec:retrieve-answer}

The two cases delivered by Section~\ref{ssec:faith-fallback} differ only in whether selected nodes carry an additional English sub-question, so we treat them under one uniform rule. A naive bilingual implementation would attach a cross-encoder reranker on top of the union of two retrievals; we avoid that by exploiting the geometry of multilingual embedding spaces, as detailed below.

Given $D \in \{D_{L}, D_{F}\}$, \textsc{Syfer} first computes a topological order
\begin{equation}
  S = (v_{1}, \ldots, v_{m}) = \mathrm{TopoSort}(D),
  \label{eq:toposort}
\end{equation}
so that every node is solved after its predecessors. The corpus $\mathcal{C}$ is encoded once with $\mathbf{e}(\cdot)$ into a single FAISS index without language partitioning, exposing the cross-lingual document overlap that the MMR pass below will exploit; a per-language index would hide this duplication and force a separate fusion step.

For a monolingual node $v_{i} = q_{i}^{L}$, retrieval uses only the target-language sub-question; for a bilingual node $v_{i} = (q_{i}^{L}, q_{j}^{\mathrm{en}})$, the English side repeats the same step and the candidate set is the union:
\begin{equation}
  R_{i} =
  \begin{cases}
    \mathrm{Retrieve}(q_{i}^{\text{filled}, L}, \mathcal{C}), & v_{i} \in V_{L}\setminus V_{\text{bi}}, \\
    \mathrm{Retrieve}(q_{i}^{\text{filled}, L}, \mathcal{C}) \cup \mathrm{Retrieve}(q_{j}^{\text{filled}, \mathrm{en}}, \mathcal{C}), & v_{i} \in V_{\text{bi}}.
  \end{cases}
  \label{eq:retrieval}
\end{equation}
The bilingual union is what creates the deduplication problem: a multilingual corpus typically stores documents whose content is identical across languages, so $R_{i}$ is dominated by parallel translations. We turn this redundancy into an asset by reordering candidates with maximal marginal relevance:
\begin{equation}
  d^{*} = \arg\max_{d \in R_{i} \setminus S_{i}}\;
  \lambda\, \mathrm{sim}(\mathbf{e}(q_{i}^{\text{filled}}), \mathbf{e}(d))
  \,-\, (1-\lambda)\, \max_{d' \in S_{i}}\, \mathrm{sim}(\mathbf{e}(d), \mathbf{e}(d')),
  \label{eq:mmr}
\end{equation}
where $S_{i}$ is the set of already selected documents and $\lambda \in [0,1]$. Because parallel translations occupy near-identical regions in the multilingual embedding space, any cross-lingual duplicate of an already-selected document is also a near-duplicate under $\mathbf{e}(\cdot)$ and is suppressed by the diversity term. Here MMR is more than a generic diversity heuristic: it acts as a parameter-free, language-agnostic deduplicator that needs neither translation alignment nor a second model.

Conditioned on $R_{i}$, the generator $M_{G}$ produces a single short answer per node, taking the bilingual pair when available so that the model can consult both formulations:
\begin{equation}
  a_{i} =
  \begin{cases}
    \mathrm{Answer}(q_{i}^{\text{filled}, L}, R_{i}), & v_{i} \in V_{L}\setminus V_{\text{bi}}, \\
    \mathrm{Answer}(q_{i}^{\text{filled}, L}, q_{j}^{\text{filled}, \mathrm{en}}, R_{i}), & v_{i} \in V_{\text{bi}}.
  \end{cases}
  \label{eq:answer}
\end{equation}
Each $a_{i}$ is substituted into placeholders $\#i$ in subsequent sub-questions. By construction, the terminal $v_{m}$ is inherited from $q_{n}^{L}$ (kept monolingual when $D_{L}$ is committed, or paired with $q_{m}^{\mathrm{en}}$ in the fallback branch), so Eq.~\eqref{eq:constraint} continues to hold for $q_{n}^{L,\text{filled}}$ and \textsc{Syfer} returns
\begin{equation}
  A = a_{m}
  \label{eq:final-answer}
\end{equation}
without an additional aggregation call over the reasoning trace, completing the synthesizer-folded pipeline.


==> tables/data_stats.tex <==
\footnotesize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.98}
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset} & \textbf{Corpus/lang} & \textbf{Corpus(9 langs)} & \textbf{Queries/lang} & \textbf{Queries(9 langs)} \\
\midrule
HotpotQA          &  9{,}811 &  88{,}299 & 1{,}000 & 9{,}000 \\
2WikiMultiHopQA             &  6{,}120 &  55{,}080 & 1{,}000 & 9{,}000 \\
MuSiQue           & 11{,}656 & 104{,}904 & 1{,}000 & 9{,}000 \\
\midrule
\textbf{Total}    & --- & \textbf{248{,}283} & --- & \textbf{27{,}000} \\
\bottomrule
\end{tabular}
